Contrastive Learning of Sociopragmatic Meaning in Social Media

Recent progress in representation and contrastive learning in NLP has not widely considered the class of \textit{sociopragmatic meaning} (i.e., meaning in interaction within different language communities). To bridge this gap, we propose a novel framework for learning task-agnostic representations transferable to a wide range of sociopragmatic tasks (e.g., emotion, hate speech, humor, sarcasm). Our framework outperforms other contrastive learning frameworks for both in-domain and out-of-domain data, across both the general and few-shot settings. For example, compared to two popular pre-trained language models, our method obtains an improvement of $11.66$ average $F_1$ on $16$ datasets when fine-tuned on only $20$ training samples per dataset.Our code is available at: https://github.com/UBC-NLP/infodcl

==> 00copy_analysis.tex <==
\textbf{Ablation Studies.} In this section, we investigate the effectiveness of each of the components in our proposed framework. To facilitate the training, we randomly extract $5$M samples from our TweetEmoji-EN dataset (with the full $1,067$ set of emojis) for these ablation experiments. Since~\citet{felbo2017using} identify a set of $64$ emojis as most influential, we also extract another random sample of $5$M tweets (Emoji64) with only these $64$ emojis to identify how our model will fare when trained only with these (vs. a model trained with the full emoji set). We evaluate our ablation models on the $16$ Twitter benchmark datasets with the same hyper-parameters we identify in Section~\ref{subsec:hyper} and report an average of five runs with different random seeds. Table~\ref{tab:ablation_avg} presents our aggregated $F_1$ scores. % for this iteration of experiments. %We also present the performance of individual task in Table~\ref{tab:ablation_full}. 
As Table~\ref{tab:ablation_avg} shows, our InfoDCL outperforms all other settings, which indicates that \textit{all} the components in our model are necessary. The results show that the most important component in our model is the emoji surrogate label prediction (SLP), which results in $1.13$ drop of average $F_1$ score when removed. Our results also show use of Emoji64 with the \textit{$64$ emoji set} suggested by~\citet{felbo2017using} instead of our \textit{full emoji label set} is sub-optimal (a drop of $0.77$ average $F_1$). This suggests that training with a large set of emoji surrogate labels helps the model capture more nuanced information relevant to social meaning. We also train an additional network to produce the weight vector, $w_i$, in LCL loss as~\citet{suresh2021not} proposed instead of using our own main model to assign this weight vector end-to-end. We observe a drop of $0.66$ averaged $F_1$ with the additional model, showing the superiority of our end-to-end approach (which is also less computational costly). Removing our epoch-wise re-pairing (EpW-RP) strategy is also valuable as removing it results in a drop of $0.59$ average $F_1$. We believe EpW-RP helps regularize our model as we dynamically re-pair an anchor with a new positive pair for each training epoch. Our results also show that our proposed CCL is as effective as LCL. Removing either of these results in $\sim 0.55$ average $F_1$ drop. We surprisingly find that the model is relatively less impacted (i.e., $\sim 0.38$ $F_1$ drop) when we remove both CCL and LCL, which implies that use of vanilla SCL loss along with other model components partially compliment both of these combined. We also adapt a simple self-augmentation method introduced by~\citet{liu2021fast} to our distant supervision setting: given an anchor $x_i$, we acquire a positive set $\{x_i, x_{m+i}, x_{2m+i}, x_{3m+i}\}$ where $x_{m+i}$ is a sample with the same emoji as the anchor,  $x_{2m+i}$ is an augmented version (applying dropout and masking) of $x_i$ and $x_{3m+i}$ is an augmented version of $x_{m+i}$. As Table~\ref{tab:ablation_avg} shows, this InfoDCL+Self-Aug method does not help our model ($0.10$ $F_1$ drop). In addition to our ablation studies, we further investigate additional issues as to how to handle surrogate labels in the context of contrastive learning. We provide this analysis in Appendix~\ref{sec:app_analysis}.


%%%%% V2 %%%%%

\vspace{-15pt}
\section{Ablation Studies and Analyses}
\label{sec:ablation_study_main}

%\subsection{Ablation Studies}\label{subsec:ablation}
\textbf{Ablation Studies.} In this section, we investigate the effectiveness of each of the ingredients of our proposed framework. To facilitate the training, we randomly extract $5$M samples from our TweetEmoji-EN dataset for our ablation experiments. %Since~\citet{felbo2017using} identify a set of $64$ emojis as most influential, we also extract another random sample of $5$M tweets (Emoji64) with only these $64$ emojis to identify how our model will fare when trained only with these (vs. a model trained with the full emoji set). 
We evaluate on the $16$ Twitter benchmark datasets with the same hyper-parameters we identify in Section~\ref{append:subsec:hyper} and report an average of five runs with different random seeds. Table~\ref{tab:ablation_avg} presents our aggregated $F_1$ scores. % for this iteration of experiments. %We also present the performance of individual task in Table~\ref{tab:ablation_full}. 
As Table~\ref{tab:ablation_avg} shows, our InfoDCL outperforms all other settings, which indicates that \textit{all} the components in our model are necessary. The results show that the most important ingredient in our model is the emoji surrogate label prediction (SLP) objective, which results in $1.13$ drop of average $F_1$ score when removed. 
%Our results also show use of Emoji64 with the \textit{$64$ emoji set} suggested by~\citet{felbo2017using} instead of our \textit{full emoji label set} is sub-optimal (a drop of $0.77$ average $F_1$). This suggests that training with a large set of emoji surrogate labels helps the model capture more nuanced information relevant to social meaning. 
We also train an additional network to produce the weight vector, $w_i$, in LCL loss as~\citet{suresh2021not} proposed instead of using our own main model to assign this weight vector end-to-end. We observe a drop of $0.66$ averaged $F_1$ with the additional model, showing the superiority of our end-to-end approach (which is also less computational costly). Our epoch-wise re-pairing (EpW-RP) strategy is also valuable, as removing it results in a drop of $0.59$ average $F_1$. We believe EpW-RP helps regularize our model as we dynamically re-pair an anchor with a new positive pair for each training epoch. Our results also show that our proposed CCL is as effective as LCL. Removing either of these results in $\sim 0.55$ average $F_1$ drop. We surprisingly find that the model is relatively less impacted (i.e., $\sim 0.38$ $F_1$ drop) when we remove both CCL and LCL, which implies that use of vanilla SCL loss along with other model ingredients partially complement both of these combined. We also adapt a simple self-augmentation method introduced by~\citet{liu2021fast} to our distant supervision setting: given an anchor $x_i$, we acquire a positive set $\{x_i, x_{m+i}, x_{2m+i}, x_{3m+i}\}$ where $x_{m+i}$ is a sample with the same emoji as the anchor,  $x_{2m+i}$ is an augmented version (applying dropout and masking) of $x_i$, and $x_{3m+i}$ is an augmented version of $x_{m+i}$. As Table~\ref{tab:ablation_avg} shows, this InfoDCL+Self-Aug method does not help our model ($0.10$ $F_1$ drop). Finally, we investigate further issues as to how to handle surrogate labels in our models. We provide this analysis in Appendix~\ref{sec:app_analysis}. %Overall, our ablation study emphasizes the crucial utility of each component of our InfoDCL model as we explained.
 \input{table_pic/ablation_avg}
%  \vspace{-5pt}
%%%%%%%%%%%%%%%%%%%%%%%%%
%We suspect that each single loss may impact the representation quality but using them together could compensate the three learning objectives, i.e., pulling samples from the same class together, distinguishing confusable samples within each class, and identifying the correlation between nuanced classes. 

 


% We train RoBERTa on $5$M data with augmented data and our framework, referring to InfoDCL+Self-Aug. We find that the self-augmentation cannot provide improvement on the downstream task performance.    

% In our method, a positive sample, $x_{m+i}$, is a tweet used as same emoji label as its anchor $x_i$. We do not use any data augmentation techniques to produce positive samples. We, then, further investigate to use a data augmentation technique to produce positive samples. We implement a simple augmentation method introduced by~\cite{liu2021fast} that creates the different view of an anchor by masking a span of tokens and masking neurons of the encoder (i.e., dropout) randomly. We apply the self-augmentation method to $x_{m+i}$ and $x_i$ and obtain two more positive samples $x_{2m+i}$ and $x_{3m+i}$, thus the positive pair is $\{x_i, x_{m+i}, x_{2m+i}, x_{3m+i}\}$. We train RoBERTa on $5$M data with augmented data and our framework, referring to InfoDCL+Self-Aug. We find that the self-augmentation cannot provide improvement on the downstream task performance. 
%%%%%%%%%%%%%%%%%%%%%%%%%

% % %\subsection{On Treating Surrogate Labels}~\label{subsec:more_analysis}
% \noindent\textbf{On Treating Surrogate Labels.} We further raise the following two questions as to how to handle surrogate labels in the context of a contrastive learning framework: \textbf{(1)} ``Should we cluster or push apart the large number of fine-grained (correlated) classes?" and ``\textbf{(2)} Can we use the emoji class embedding (EC-Emb) for corpus-level weighting?". For space limitation, we provide the complete analysis related to these two questions in Appendix~\ref{sec:app_analysis}.

\input{qualitative}

% \chiyu{t-sne visualization and clustering}




==> contrastive.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Contrastive Learning}\label{sec:cl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Contrastive learning (CL) aims at bringing semantic representations of instances of a given class (e.g., \textit{positive pairs} of the same objects in images or same topics in text) closer and representations of negative class(es) instances farther away~\cite{fang2020cert,liu2021fast,gao2021simcse}. %Formally, CL optimizes for two key properties: \textit{alignment} that measures how close are the representations of the positive pairs and \textit{uniformity} that measures how well the representations are uniformly distributed~\cite{wang2020understandingcl}. 
One way most CL frameworks differ is how positive pairs are defined. In \textit{self-supervised contrastive learning} (SSCL), a positive pair is typically formed by pairing an anchor sample with its transformation (e.g., cropping an image~\cite{cubuk2018autoaugment, caron2020unsupervised, chen2020simple}, replacing some words in a sentence with their synonyms~\cite{wang2021cline}). On the other hand, \textit{supervised contrastive learning} (SCL) not only uses the transformation of an anchor but also samples from the same class as its positive samples exploiting gold-labeled data. Existing SCL frameworks~\cite{gao2021simcse, khosla2020supervised, gunel2020supervised, suresh2021not} suffer from \textbf{two major drawbacks}. The \textbf{first drawback} is SCL's dependence on task-specific labeled data (which is required to identify positive samples in a batch). Recently,~\citet{zheng2021weakly} introduced a \textit{weakly-supervised contrastive learning} (WCL) objective for computer vision, %based on labels acquired using graph-based clustering approach from heavily augmented training data. 
which generates a similarity-based \textit{1}-nearest neighbor graph in each batch and assigns weak labels for samples of the batch (thus clustering vertices in the graph). %However, it is suboptimal that samples are cluster in batch and the clusters cannot reflect the global similarity between samples. }
It is not clear, however, how much an WCL method with augmentations akin to language would fare for NLP. We propose a framework that does not require model-derived weak labels, which outperforms a clustering-based WCL approach. The \textbf{second drawback} with SCL is related to how negative samples are treated.~\newcite{gao2021simcse,khosla2020supervised,gunel2020supervised} treat all the negatives equally, which is sub-optimal since confusable negatives should be more informative. To rectify this,~\newcite{suresh2021not} introduce a \textit{label-aware contrastive loss} (LCL) where they feed the anchor sample to a task specific model and assign higher weights to confusable negatives based on this model's confidence on the class corresponding to the negative sample. LCL, however, is both \textbf{narrow} and \textbf{costly}. It is narrow since it exploits \textit{task-specific} labels. We fix this by employing surrogate labels generalizable to \textit{all} sociopragmatic meaning rather than particular tasks. In addition, LCL is costly since it requires an auxiliary task-specific model to be trained with the main model. Again, we fix this issue by introducing a \textit{light} LCL framework (\textbf{LCL-LiT}) where we use our main model, rather than an auxiliary model, to derive the weight vector $w_{i}$ from our main model through an additional loss (i.e., weighting is performed end-to-end in our main model). A further issue with LCL is that it \textbf{only considers instance-level information} to capture relationships between different classes. In comparison, we introduce a novel corpus-aware contrastive loss that overcomes this issue. We now introduce our new framework. %\chiyu{Furthermore, \cite{wang-2021-understanding} identify a uniformity-tolerance dilemma of contrastive learning, the excessively pursuing to uniformity result that the contrastive loss intolerates to semantically similar samples, which may destroy its underlying semantic structure and be harmful to downstream tasks. In this work, we introduce an effective contrastive loss that takes into account corpus-level information (Section~\ref{subsec:ccl}) and preserve the semantic structure in representations. }


%The \textbf{third drawback} with existing CL methods in general is related to the uniformity-tolerance dilemma identified by~\cite{wang-2021-understanding}: In their attempt to solve anisotropy, CL methods excessively pursue uniform distributions of representations that results in a loss intolerant to class-wise semantically similar samples.\footnote{In other words, the loss becomes intolerant to  self-similarity Semantically similar means similar to self in the case of SSCL and similar to other samples in the same class in the case of SCL.} This, in turn, may destroy the underlying semantic structure of representations and cause harm to downstream task performance. 







==> multi-lingual.tex <==
\subsection{Multi-lingual Tasks}%\label{subsec:multi-ling}
\input{table_pic/multi-lingual}
We also investigate the effectiveness of our proposed model on multi-lingual tasks. Table~\ref{tab:multi-lingual} presents the performance on nine downstream tasks in three different languages. We continue training XLM-R with our proposed objectives. We experiment three settings: (1) English only: training on 1M English tweets and evaluating on nine multi-lingual tasks, (2) Target mono-lingual: training on 1M mono-lingual tweets in the target language~\footnote{For the Italian model, we only obtain 0.5M tweets for continuing training.} and evaluating on tasks of the target language, (3) Multi-lingual: training on $4.5$M tweets in four language (i.e., Arabic, Italian, Spanish, and English) and evaluating on nine multi-lingual tasks. We still use the NPMI weighting matrix generated from English tweets in these experiments.~\footnote{We will explore the generating NPMI weighting matrix from mutli-lingual data in the future work.} Table~\ref{tab:multi-lingual} shows that our models outperform the original XLM-R on all the tasks and obtains the improvement with $1.44$ and $0.85$ average $F_1$ across nine tasks under multi-lingual and target mono-lingual settings respectively. Training on English mono-lingual data helps four tasks but cannot benefits all nine non-English tasks on average. Compare to previous SoTA models, our proposed methods outperform on six out of nine tasks.~\footnote{For Emo-es\textsubscript{Moham}, we use fine-tuning XLM-R as SoTA model because we convert the intensity regression task to a emotion classification.} These results demonstrate that our methods is not only task-agnostic but also language-agnostic. 

==> table_pic/gold_data_emoji.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\small
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Task}}            & \multicolumn{1}{c}{\textbf{Train}} & \multicolumn{1}{c}{\textbf{Dev}} & \multicolumn{1}{c}{\textbf{Test}} \\ \midrule
Crisis\textsubscript{Oltea} & 0.01                               & 0.02                             & 0.00                              \\
Emo\textsubscript{Moham}    & 11.39                              & 27.81                            & 23.43                             \\
Hate\textsubscript{Was}     & 2.23                               & 2.03                             & 2.76                              \\
Hate\textsubscript{Dav}     & 0.00                               & 0.00                             & 0.00                              \\
Hate\textsubscript{Bas}     & 6.50                               & 1.50                             & 11.57                             \\
Humor\textsubscript{Mea}    & 0.55                               & 0.00                             & 1.00                              \\
Irony\textsubscript{Hee-A}  & 10.58                              & 10.94                            & 11.22                             \\
Irony\textsubscript{Hee-B}  & 10.58                              & 10.94                            & 11.22                             \\
Offense\textsubscript{Zamp} & 11.43                              & 10.88                            & 13.37                             \\
Sarc\textsubscript{Riloff}  & 5.38                               & 3.39                             & 4.52                              \\
Sarc\textsubscript{Ptacek}  & 4.34                               & 4.36                             & 4.92                              \\
Sarc\textsubscript{Rajad}   & 16.94                              & 18.01                            & 17.10                             \\
Sarc\textsubscript{Bam}     & 8.47                               & 8.29                             & 9.64                              \\
Senti\textsubscript{Rosen}  & 0.00                               & 0.00                             & 6.59                              \\
Senti\textsubscript{Thel}   & 0.00                               & 0.00                             & 0.00                              \\
Stance\textsubscript{Moham} & 0.00                               & 0.00                             & 0.00                              \\ \midrule
Emotion\textsubscript{Wall} & 0.00                               & 0.00                             & 0.00                              \\
Emotion\textsubscript{Dem}  & 0.00                               & 0.00                             & 0.00                              \\
Sarc\textsubscript{Walk}    & 0.00                               & 0.00                             & 0.00                              \\
Sarc\textsubscript{Ora}     & 0.00                               & 0.00                             & 0.10                              \\
Senti-MR                                     & 2.01                               & 1.76                             & 1.84                              \\
Senti-YT                                     & 0.00                               & 0.00                             & 0.00                              \\
SST-5                                        & 0.00                               & 0.00                             & 0.00                              \\
SST-2                                        & 0.00                               & 0.00                             & 0.00                              \\ \midrule
Emo\textsubscript{Mag}      & 16.58 & 25.27 & 25.40 \\
Emo\textsubscript{Bian}     & 27.62 & 28.43 & 32.84 \\
Emo-es\textsubscript{Moham} & 23.67 & 21.94 & 22.71 \\
Hate\textsubscript{Bos}     & 1.93  & 1.67  & 1.50  \\
Hate-es\textsubscript{Bas}  & 11.07 & 10.00 & 7.63  \\
Irony\textsubscript{Ghan}   & 8.62  & 9.68  & 7.95  \\
Irony\textsubscript{Cig}    & 1.68  & 2.01  & 5.50  \\
Irony\textsubscript{Ort}    & 11.94 & 15.00 & 10.00 \\
Offense\textsubscript{Mub}  & 38.79 & 36.50 & 38.75 \\ \bottomrule
\end{tabular}
\caption{Percentage of samples of downstream tasks containing emojis. }\label{tab:labeled_emoji}
\end{table}

==> table_pic/senteval_hashtag.tex <==
\begin{table*}[!ht]
\centering
\tiny
\begin{tabular}{@{}lcccccccccc|cc@{}}
\toprule
\textbf{Task} & \textbf{RB} & \textbf{MLM} & \textbf{H-MLM} & \textbf{SLP} & \textbf{Mir-B} & \textbf{Sim-S} & \textbf{Sim-D} & \textbf{WCL} & \textbf{DCL}   & \textbf{Ours-R} & \textbf{BTw}   & \multicolumn{1}{l}{\textbf{Ours-B}} \\ \midrule
STS12         & 15.88       & 32.26        & 20.45          & 27.25        & 61.15          & \textbf{61.98} & 34.96          & 17.54        & 37.69          & 37.02           & 29.20          & \textbf{33.79}                      \\
STS13         & 38.11       & 54.13        & 44.32          & 39.67        & \textbf{71.65} & 69.85          & 42.95          & 34.19        & 42.52          & 41.23           & 36.26          & \textbf{40.69}                      \\
STS14         & 28.58       & 41.92        & 33.34          & 23.93        & \textbf{67.55} & 64.41          & 29.47          & 22.78        & 28.61          & 28.48           & \textbf{33.76} & 29.98                               \\
STS15         & 40.22       & 60.11        & 47.44          & 35.81        & \textbf{76.55} & 75.76          & 42.34          & 48.19        & 40.37          & 41.48           & \textbf{49.19} & 46.28                               \\
STS16         & 50.12       & 66.57        & 59.95          & 46.37        & \textbf{76.57} & 74.18          & 48.06          & 31.50        & 47.74          & 49.38           & 46.99          & \textbf{47.67}                      \\
SICK-R        & 62.54       & 64.02        & 62.12          & 46.32        & \textbf{66.60} & 66.09          & 57.23          & 47.82        & 56.25          & 53.94           & 48.76          & \textbf{57.49}                      \\
STS-B         & 46.63       & 57.39        & 46.20          & 33.20        & \textbf{72.92} & 71.11          & 37.40          & 37.95        & 36.87          & 38.05           & \textbf{38.24} & 37.08                               \\ \cdashline{1-13}
Average       & 40.30       & 53.77        & 44.83          & 36.08        & \textbf{70.43} & 69.05          & 41.77          & 34.28        & 41.44          & 41.37           & 40.34          & \textbf{41.85}                      \\ \midrule
MR            & 75.92       & 78.11        & 78.76          & 84.21        & 78.01          & 76.06          & \textbf{85.24} & 75.16        & 85.08          & 85.14           & 79.58          & \textbf{84.10}                      \\
CR            & 69.59       & 74.89        & 83.63          & 89.38        & 83.92          & 81.51          & 89.59          & 78.99        & 89.56          & \textbf{89.62}  & 80.82          & \textbf{89.46}                      \\
SUBJ          & 91.50       & 91.33        & 92.21          & 93.17        & 92.21          & 91.45          & 94.64          & 92.77        & \textbf{94.73} & 93.81           & 93.03          & \textbf{94.54}                      \\
MPQA          & 73.75       & 80.62        & 78.03          & 86.25        & 85.69          & 84.95          & \textbf{87.29} & 85.95        & 86.86          & 86.18           & 71.78          & \textbf{87.91}                      \\
SST2          & 82.81       & 84.95        & 87.97          & 89.57        & 82.98          & 81.05          & 89.84          & 78.91        & 90.01          & \textbf{90.50}  & 86.66          & \textbf{90.77}                      \\
SST5          & 38.46       & 42.17        & 42.49          & 49.23        & 46.11          & 44.52          & 50.77          & 42.81        & \textbf{51.36} & 50.23           & 43.71          & \textbf{50.86}                      \\
TREC          & 61.40       & 74.60        & 65.40          & 73.00        & \textbf{86.80} & 85.60          & 79.20          & 86.40        & 78.00          & 81.00           & 80.80          & \textbf{87.00}                      \\
MRPC          & 71.42       & 74.09        & 70.03          & 68.99        & \textbf{74.84} & 74.09          & 69.33          & 69.68        & 69.33          & 67.54           & \textbf{72.35} & 69.86                               \\ \cdashline{1-13}
Average       & 70.61       & 75.10        & 74.82          & 79.23        & 78.82          & 77.40          & \textbf{80.74} & 76.33        & 80.62          & 80.50           & 76.09          & \textbf{81.81}                      \\ \bottomrule
\end{tabular}
\caption{Evaluate hashtag-based models on SentEval.}\label{tab:senteval_hashtag}
\end{table*}
